Combining Emulation and Simulation to Evaluate a Near Memory Key/Value Lookup Accelerator

Processing large numbers of key/value lookups is an integral part of modern server databases and other "Big Data" applications. Prior work has shown that hash table based key/value lookups can benefit significantly from using a dedicated hardware lookup accelerator placed near memory. However, previous evaluations of this design on the Logic in Memory Emulator (LiME) were limited by the capabilities of the hardware on which it was emulated, which only supports a single CPU core and a single near-memory lookup engine. We extend the emulation results by incorporating simulation to evaluate this design in additional scenarios. By incorporating an HMC simulation model, we design optimizations that better mitigate the effects of the HMC closed page policy and that better utilize the HMC's parallelism, improving predicted performance by an order of magnitude. Additionally, we use simulation to evaluate the scaling performance of multiple near-memory lookup accelerators. Our work employs an open source emulator LiME, open source simulatation infrastructure SST, and the open source HMC-Sim simulator.

==> results.tex <==

\section{Experimental evaluation}
\label{sec:experiments}
\subsection{Emulator}
The prototype hardware lookup accelerator has been implemented in 
LiME \cite{g114,emuurl}, a hardware/software infrastructure that uses the 
Xilinx ZC706 development board with Zynq 7045
System-on-Chip. The Zynq has two 32-bit ARM cores, a hard 32-bit
memory controller, other I/Os, and  programmable logic. The
development board has two
on-board DDR3 memories and external I/O such as PCIe and Ethernet. The infrastructure supports
emulation of the key/value table software and hardware components. For
the lookup accelerator experiment, the
software runs ``bare metal'' on an ARM core to populate the table, generate the query workload,
and communicate with the hardware lookup accelerator to process block
get requests. The lookup accelerator is mapped to FPGA logic in the programmable
logic portion of the chip. 

The ARM processor cores have
separate L1 (32\,KB, 4-way set-associative instruction and data) and
shared L2 (512\,KB, 8-way set-associative) caches. A 1\,GB 32-bit wide
DDR3 memory is used to hold application code and
data. A second DDR memory connected to the
programmable logic is used by the emulator to hold memory traces. % In our
% experiments, the CPU software runs ``bare metal'' without an Operating
% System, allowing measurement of the application in isolation and as
% importantly, giving the application nearly the entire 1\,GB memory.

The ARM cores can run at a clock frequency ranging from 1\,MHz to
800\,MHz. For these experiments, the ARM runs at 128.6\,MHz to achieve
the emulated CPU frequency of 2.57\,GHz. The lookup accelerator runs at an
emulated 1.25\,GHz. The emulation infrastructure
contains programmable delay units in the FPGA fabric to emulate
different memory latencies. The delay units are programmable at a
range of 0--262\,us in 0.25\,ns increments. The emulated memory
subsystem has multiple memory channels and is capable of accepting up
to 16 concurrent memory requests and multiple access widths. In this
evaluation, a 32-byte access width is used from the CPU and up to
a 128-byte width is used from the accelerator. 

When trace capture is invoked by software running on the ARM
processor, the emulator copies memory requests to the second DDR
memory while simultaneously routing them through the delay units to
the first memory. The stored memory event includes source of request
(CPU or accelerator), type of request (Read or Write), access width,
and time stamp. Typically trace capture is turned during execution of
a region of interest. These captured traces were used to help validate
the simulator model.

\subsection{Experiment design}
Our experiment fills the key/value table with a scientific data
set consisting of k-length genomic sequences, i.e. k-mers. A 32 million entry table is
the largest size that fits in the emulator's program memory. In open
addressing, the entire table is allocated on initialization. Our
experiments fill the table to varying degrees, which is the table's
{\em load factor}. The load factor determines the probe sequence
length, which in turn determines the lookup accelerator's bandwidth
requirement. 

A query may result in the key being found or that the requested item
is not present in the table. The {\em hit ratio} determines the
probability that the item is in the table. A low hit ratio results in
the longest probe sequence length being searched, whereas a high hit ratio
means the item is likely to be found with average case search length.
In our design, the lookup accelerator always scans up to the longest
probe sequence length in the table, but software can short circuit a search as soon as the
item is found. By measuring performance at different hit ratios, the
relative advantages of hardware acceleration vs. software are
illuminated.

Another differentiating factor of table lookup is a key's popularity,
i.e. how often is the same item looked up. For some applications such
as social media \cite{Atikoglu:2012}, a particular topic or URL may dominate searches for a
period of time, whereas other use cases may have a more random key
{\em repeat} frequency. The high repeat frequency scenario is modeled by a
zipfian distribution, and the random case uses the uniform
distribution. 

By employing a high quality hash algorithm we effectively randomize
the key's hash index. We sweep the load factor across a large range,
resulting in a full range of probe sequence lengths. The key repeat
frequency models two representative query patterns.
These techniques enable us to model a
large range of workloads using the single k-mer data set.

A final parameter most relevant to near memory processing is the
memory {\em latency}. Memory latency may vary from 10\,ns for
SRAM to microseconds for slower memory technology. The experiments
use two different frequency groups. The 85\,ns read with 106\,ns write
case models HMC/HBM memory latency as measured on a Gen 1 4\,GB HMC with
128 byte packets. The
200\,ns read with 400\,ns write case models the faster proposed SCM
latency projections.

The query block size is 1024 keys.
Table \ref{tab:paramstab} summarizes the parameters that are swept in this
experimental evaluation.


\begin{table}
\begin{center}
    \begin{tabular}{|c||c|c|c|c|}
    \hline
     \multicolumn{2}{|c||}{load factor} & \multicolumn{3}{|c|}{10\%--90\%} \\ \hline 
    \multicolumn{2}{|c||}{hit  ratio} & 10\%& 50\%& 90\% \\ \hline 
    repeat & \multicolumn{2}{|c|}{uniform} & \multicolumn{2}{|c|}{zipf} \\ \hline 
    latency & \multicolumn{2}{|c|}{85R/106W} &\multicolumn{2}{|c|}{200R/400W}  \\ \hline 
    \multicolumn{3}{|c||}{query block size} & \multicolumn{2}{|c|}{1024 keys}  \\ \hline 
    \end{tabular}
    \caption{\label{tab:paramstab} Lookup workload parameters }
\end{center}
 \end{table}

In the evaluation, we compare three lookup algorithms: 
\begin{itemize}
\item ``Accel,''  the near memory
hardware lookup accelerator as described in Section \ref{sec:hworg}, 
\item ``Soft,'' a software version of the hardware lookup algorithm
  using the identical open addressing and hash algorithm.  Unlike the
  hardware, the software algorithm terminates probe sequence search as
  soon as a key has been found.
\item ``STL,'' a hash table that uses the Standard Template Library (STL)
  unordered map.
\end{itemize}

Since STL uses more memory than Soft, the load
factor could only
be measured up to 70\% for STL.
Timings are measured for the batch get operation as issued by the CPU
core. The software runs on the emulated 32-bit 2.57\,GHz ARM
processor.

\subsection{Experiment findings}


\begin{figure}
\begin{centering}
\includegraphics[width=2.95in]{results/arm32-mem-uniform-hit90}
\par\end{centering}
\caption{\label{fig: arm32-mem-uniform-hit90} Lookup rates of HMC using uniform
key query repeat frequency at 90\% hit rate}
\end{figure}
\begin{figure}
\begin{centering}
\includegraphics[width=2.95in]{results/acc-mem-zipf-hit90}
\par\end{centering}
\caption{\label{fig: acc-mem-zipf-hit90} Lookup rates of HMC and SCM using zipfian
key query repeat frequency at 90\% hit rate}
\end{figure}

Results from running the k-mer query workload on the emulated near memory
lookup accelerator and associated CPU core indicate significant
performance benefit to the proposed lookup accelerator. 
Figure \ref{fig: arm32-mem-uniform-hit90} graphs the effect of
increasing hash table occupancy (i.e. load factor) on the lookup rate for the three
versions. For a sparsely filled table, hardware acceleration gives 64.3\,M
lookups/s. The trend line decreases linearly with increasing
occupancy, with 9.13\,M lookups/s at 90\% load factor. Both software
versions show slightly decreasing performance
ranging from 5\,M at light occupancy to 2.6\,M at 90\% for Soft and
slightly less for STL. The graph shows a workload with uniform key
query frequency. Zipfian is not shown since its trend line is nearly
identical to uniform. Hardware speed for zipfian is the same as for
uniform since the hardware pipeline scans the entire max probe
sequence length. Software lookup rate for zipfian goes from a high of 5.8\,M
lookups/s at 10\% load factor to 4.76\,M at 90\% load factor.

The complete suite of experiments was also done using the SCM latency
profile. Figure \ref {fig: acc-mem-zipf-hit90} compares HMC vs. SCM
performance on the hardware accelerated lookup workload using a
zipfian key frequency and 90\% hit rate. While using HMC results in
more than double the query performance at a 10\% load, HMC performance
benefit decreases more steeply than SCM. At the 90\% load factor, the
two converge. At 90\% load factor, the long probe sequence length
results in optimal sequential DMA bursts that maximize memory
bandwidth, shifting the bottleneck to the hardware accelerator
pipeline.

The speedup trends comparing uniform and zipfian key distribution in
HMC-like memory are shown in
Figure \ref{fig:speedup-arm32-acc-mem-uz-hit90}. They both follow the
hardware accelerator's lookup rate as the load factor
increases. The uniform key repeat pattern starts at the high of 12.8X over software at low
occupancy, it decreases linearly to 3.5X at the 90\% load
factor. Zipfian shows a similar trend, but has slightly less speedup,
showing the benefit of CPU cache for repeat queries. It has speedup of
10.2X at 10\% load factor trending down to speedup of 2.9X at the
highest load factor.

\begin{figure}
\begin{centering}
\includegraphics[width=2.95in]{results/speedupvsloadfactor-zipf-uniform}
\par\end{centering}
\caption{\label{fig:speedup-arm32-acc-mem-uz-hit90} Speedup on HMC
  comparing uniform and zipfian
key query repeat frequency at 90\% hit rate}
\end{figure}


The chart in Figure \ref{fig:speedup-arm32-acc-scm-uz-hit90} shows the
same comparison with SCM. Speedup is lower than with HMC-like
memory at low load factor, but is greater as the table occupancy increases.

Figures \ref{fig:speedup-mem-z10-90} and \ref{fig:speedup-scm-z10-90}
quantify the speedup differences between zipfian query workloads that
usually don't find the key (10\% hit rate) and those that almost always find the
key (90\% hit rate). We sweep the load factor parameter to analyze performance as the
hash table gets more full, which results in increasing probe sequence
length. 

\begin{figure}
\begin{centering}
\includegraphics[width=2.95in]{results/speedupvsloadfactor-zipf-uniform-scm}
\par\end{centering}
\caption{\label{fig:speedup-arm32-acc-scm-uz-hit90} Speedup on SCM
  comparing uniform and zipfian
key query repeat frequency at 90\% hit rate}
\end{figure}

The hardware accelerator query throughput tracks load factor,
as the hardware scans the entire max probe sequence length for each
query. However, software query rate varies since the query can
complete as soon as the key is found. The charts show that at a low load factor, hit rate doesn't
affect speedup, which is around 10X for both cases. As the load factor
increases, speedup for both hit rates decreases. However, the 10\% hit
rate speedup decreases much less at higher load factor, and the
speedup even increases a significant amount at low hit rate and high
load factor. The profiles for SCM show an even more pronounced
increase in speedup at high load factor for the 10\% hit rate and high
load factor. We attribute the upward trend of the speedup curve for
low hit rate to the fact that at high load factor, the probe sequence
length is longer and software must scan the whole sequence to
determine the key doesn't exist in the table. The high latency of SCM
pushes that trend even more.



Our analysis has swept the critical factors affecting hash table
performance applicable across a very wide range of use cases and found
that in every case, the near memory hardware hash table lookup
accelerator is significantly faster, from a maximum of 12.8X for a
10\% load factor with 90\% hit rate on a uniform key query frequency
in HMC-like memory, to a minimum of 2.9X with 90\% load factor and
90\% hit rate with a zipfian key frequency in HMC-like memory. Overall
the speedup is higher in SCM for the most challenging workloads, where
the latency of bring the SCM cache lines to the CPU affect CPU
performance.

\subsection{Discussion and future experiments}

\begin{figure}
\begin{centering}
\includegraphics[width=2.95in]{results/speedup-arm32-acc-mem-zipf-hit10-90}
\par\end{centering}
\caption{\label{fig:speedup-mem-z10-90} Speedup comparison in HMC with
  zipfian
key query repeat frequency at 10\% and 90\% hit rates}
\end{figure}

\begin{figure}
\begin{centering}
\includegraphics[width=2.95in]{results/speedup-arm32-acc-scm-zipf-hit10-90}
\par\end{centering}
\caption{\label{fig:speedup-scm-z10-90} Speedup comparison in SCM with
  zipfian
key query repeat frequency at 10\% and 90\% hit rates}
\end{figure}

We first note that we implement a bulk get operation: the overhead of
synchronization with the accelerator is amortized by having each
request process a 1\,K block of queries. This approach is suitable for data
analytics and for streaming network requests. We analyze 8 byte keys and
4 byte values, well suited to indexing schemes that hash the
variable length key into a fixed size and use the value field as a
pointer to the actual key and value.

These results have been measured in the FPGA emulator's
environment. The lookup benchmark software runs on a physical ARM A9 core and
the hardware pipeline runs on the FPGA fabric. The ARM clock frequency
and the FPGA design clock frequency are set to emulate a 2.57\,GHz clock
on the ARM core and 1.25\,GHz clock for the entire hardware
pipeline. Memory latency is emulated by setting delay unit
parameters. The emulation environment is 100\%
accurate for these parameters. It is also highly
efficient, with a slowdown over real time of only 20, in contrast to
software simulation of CPU, cache, and memory which have thousands of
times slowdown.

A limitation of our approach is that CPU microarchitecture and cache
hierarchy are fixed. The effects of modifications to the instruction
set, microarchitecture, or cache hierarchy cannot be explored. For
example, cache flush and invalidate incur substantial overhead. It
would be illuminating to explore the tradeoffs of introducing
region-based cache-memory synchronization. Running the query workbench
in a full software CPU simulator such as Gem5 \cite{gem5} and an HMC
or HBM simulator e.g. \cite{leidelhmc,Jung:2016} would enable these
aspects to be studied.

Our specific platform, a Zynq development board, is attractive from
the cost viewpoint, but it limits us to a table under 1\,GB. Porting the
emulator to a platform with more external memory would allow
evaluation with larger workloads.

The hardware load store units use the hashed keys as offsets from the
base 
hash table address to form the final address issued to the memory. The hardware does not perform virtual-to-physical
translation, and in these experiment the entire hash table
is in a physically continuous region of memory. Other researchers have
designed address translation within the memory with IOMMU-like schemes
or optimized page table translation as in
\cite{hsieh2016accelerating}. However, it is difficult to make a
generic memory-based page table translation mechanism independent of a
specific CPU and OS. For an open addressing hash table in which the
entire table is allocated at the outset, it is easier to allocate a
contiguous physical  than with linked data structures.

The study has focused on a single CPU core and a single
pipeline. Previously we have taken a single core
memory trace and multiplexed it to simulate multiple independent
concurrent threads. The multiplexed traces were run on an HMC
\cite{g112}.  While the multiplexed trace exhibits a specific memory request order
that might be different in a true concurrent execution in which the
cores shared cache, it nevertheless can illuminate behavior of the
memory interface under load using application-specific access
patterns. We hope to perform a similar study for this workload.

Finally, this study has focused on throughput performance. We plan in
the future to analyze the energy profile of the hardware/software approach. 

\section{Conclusions}

The key/value store is perhaps the most prevalent function in use
today to support data analytics, and therefore may have sufficient
commercial interest to overcome the expense of near memory
hardware. To quantify potential benefit of near memory hardware
accelerated key/value store lookup, we have designed and prototyped a
lookup accelerator. Our design optimizes for streaming memory requests
by building an open addressing hash table to implement the key/value
store.

The accelerator uses simple hardware primitives including
load-store units for gather operations, hash units, comparators,
splitters, and fifos. The hash unit used in these studies is the
hardware implementation of one of the best, hardware friendly hash
functions published. The building blocks have been composed in a
synchronous 
high performance pipeline capable of delivering a result every few clock
cycles.

The accelerator has been evaluated with a query workload sweeping a
wide range of parameters and shown excellent speedup on both HMC/HBM
memory and storage class memory. Our future work
includes evaluation with additional CPU and cache alternatives and
concurrent workloads.
